Adversarial Example Games

The existence of adversarial examples capable of fooling trained neural network classifiers calls for a much better understanding of possible attacks to guide the development of safeguards against them. This includes attack methods in the challenging non-interactive blackbox setting, where adversarial attacks are generated without any access, including queries, to the target model. Prior attacks in this setting have relied mainly on algorithmic innovations derived from empirical observations (e.g., that momentum helps), lacking principled transferability guarantees. In this work, we provide a theoretical foundation for crafting transferable adversarial examples to entire hypothesis classes. We introduce Adversarial Example Games (AEG), a framework that models the crafting of adversarial examples as a min-max game between a generator of attacks and a classifier. AEG provides a new way to design adversarial examples by adversarially training a generator and a classifier from a given hypothesis class (e.g., architecture). We prove that this game has an equilibrium, and that the optimal generator is able to craft adversarial examples that can attack any classifier from the corresponding hypothesis class. We demonstrate the efficacy of AEG on the MNIST and CIFAR-10 datasets, outperforming prior state-of-the-art approaches with an average relative improvement of $29.9\%$ and $47.2\%$ against undefended and robust models (Table 2 & 3) respectively.

==> MAIS2020/expe.tex <==
\xhdr{Experiments}
We investigate the application of our AEG framework to produce adversarial examples against classifiers trained on the MNIST and CIFAR-10 datasets.
% \footnote{Code: \url{https://github.com/hugobb/NoBoxAttack}}
Through our experiments we seek to answer the following questions: 
% \begin{enumerate}[label=({\bf Q\arabic*}), leftmargin=28pt, topsep=2pt, itemsep=2pt, parsep=2pt]
% \item
 \textbf{(Q1) Known-Architecture Attacks.} Can we effectively generate attacks when we only know the architecture (but not the parameters) of the target model? In this case, the architecture specifies the hypothesis class of the target model, but have no access to the target model itself. (Table~1)
%  \item
\textbf{(Q2) Architecture Transfer Attacks.} Can we generate effective attacks even when the representative classifier ($f_c$) that we use during optimization implements a distinct architecture from the target model ($f_t$)? In this experiment, we do not even know the specific architecture of the target model and must implicitly attack a much larger hypothesis class. (Table~2)
%  \item
% \textbf{(Q3) Attacking Robust Classifiers.} Can we successfully attack robustified classifiers \cite{madry2017towards,tramer2017ensemble}? Under standard {\em PGD adversarial training} \cite{madry2017towards} this corresponds to a worst-case setting for our attacker. While for {\em ensemble adversarial training} \cite{tramer2017ensemble} this involves injecting adversarial examples from other architectures, thus expanding the hypothesis class of the target model. %since we must fool a model that we have no interactive access to and that has been trained to be robust against adversarial attacks. 
% \end{enumerate}
Throughout our experiments we rely on four representative blackbox attack strategies adapted to the NoBox setting: the Momentum-Iterative Attack (MI-Attack) \citep{dong2018boosting}, the Input Diversity  (DI-Attack)\citep{xie2019improving}.
For fair comparison, we inherit all hyperparameter settings from their respective papers and note that certain attacks are architecture dependent such as the SGM-attack, which is only permitted in architectures that contain skip connections. 
We perform all attacks, including baselines, on test datasets $\mathcal{D}$ of size $256$ and with respect to the $\ell_{\infty}$ norm constraint with $\epsilon=0.3$ for MNIST and $\epsilon=0.03125$ for CIFAR-10.


% \subsection{Experimental Setup}
% \label{sub:experiments}


% \xhdr{Model details}
% We train both the generator ($g$) and representative classifier ($f_c$) using stochastic gradient descent-ascent with the ExtraAdam optimizer~\citep{gidel2019variational} and held out target models, $f_t$, are trained offline using SGD with Armijo line search \cite{vaswani2019painless}.
% Full details of our model architectures employed in our AEG framework, as well as details on hyperparameter tuning, can be found in Appendix \S{\ref{app:architecture}}.
% In order to generate adversarial perturbations over images that obey $\epsilon$-ball constraints, we employ a scaled tanh output layer to scale the output of the generator to $(0,1)$, subtract the clean images, and finally apply an elementwise multiplication by $\epsilon$. Note that---in addition to training against $f_c$---in practice we also find it beneficial to include a pre-trained and fixed classifier $f_s$ as a mechanism to incorporate prior knowledge during AEG optimization. 
% Intuitively, $f_s$ plays an analogous role as the representative classifier $f_c$ but is pre-trained on $\mathcal{D}_\textrm{train}$ and remains fixed during optimization, providing additional gradient signal and a source of stability during the optimization process. 
% %To optimize in our AEG framework, we initialize the representative classifier $f_c$ with random initializing using the architecture of a source model. Using the architecture of a source model, empirically we find that using another pretrained classifier $f_s$ in tandem with $f_c$ leads to stronger attacks. We note however, that this pretrained source model $f_s$ remains fixed throughout the entire training of the generator and only $f_c$ is updated. 

% \xhdr{Baselines}
% Throughout our experiments we rely on four representative blackbox attack strategies adapted to the NoBox setting: the Momentum-Iterative Attack (MI-Attack) \cite{dong2018boosting}, the Input Diversity  (DI-Attack)\cite{xie2019improving}, the Translation-Invariant (TID-Attack) \cite{dong2019evading} and the Skip Gradient Method (SGM-Attack) \cite{wu2020skip}.
% For fair comparison, we inherit all hyperparameter settings from their respective papers and note that certain attacks are architecture dependent such as the SGM-attack, which is only permitted in architectures that contain skip connections. 


% \subsection{Results}
% We now address the core experimental questions (\textbf{Q1}-\textbf{Q3}), highlighting the performance of adversarial examples crafted using our AEG framework.

% \xhdr{Q1: Known-Architecture Attacks}

% These results and samples of adversarial examples generated by $g$ are provided in Appendix \ref{appendix:qual_results}.

\label{q1}
\begin{table}[h]
    \begin{small}
    \vspace{-1mm}
    \centering
            \begin{tabular}{cccccc}
            \toprule
                   Dataset & MI-Attack & DI-Attack  &  AEG (Ours) \\
                    \midrule
                    MNIST  & $93.7 \pm 1.1 $ & \textbf{95.9 $\pm$ 1.6}  & \textbf{96.1$\pm$ 2.3} \\
                    \midrule
                    CIFAR-10  & \textbf{99.9 $\pm$0.1} & \textbf{99.9 $\pm$ 0.1} &  $98.5 \pm 0.7$ \\
            \bottomrule
            \end{tabular}
                \label{q2_table}
            \caption{
            We evaluate the ability of AEG adversarial examples to attack different models from a given hypothesis class, specified by a neural network architecture.
Specifically, we train $20$ LeNet \cite{lecun2015lenet} classifiers on MNIST \cite{lecun-mnisthandwrittendigit-2010} and $10$ classifiers using the Wide ResNet architecture \cite{zagoruyko2016wide} for CIFAR-10 \cite{krizhevsky2014cifar}. 
% To evaluate the baselines, we randomly select one trained classier as the source model that the baselines attack while the remaining classifiers are taken to be held out target models. 
%In addition to NoBox adversary baselines, we also compare our approach with strong whitebox and blackbox query baselines adapted to the NoBox setting \cite{croce2019minimally,croce2020reliable,li2019nattack,andriushchenko2019square,tu2018autozoom}, these results are outlined in Appendix A.  
% Our results in this setting are summarized in Table 1. As can be observed, adversarial examples found using AEG exhibit the highest transferability to other MNIST classifiers. On CIFAR-10 we find that AEG adversarial examples are competitive with the baselines (i.e., within $1.4\%$), though some baselines achieve near perfect transfer in this setting.
%We hypothesize that there is more diversity in the trained 
%We hypothesize that decision boundaries learned by these functions are very similar and thus effectively whitebox attack success rates can be obtained.
% In addition to NoBox baselines, we also compare our approach with strong whitebox and blackbox query baselines adapted to the NoBox setting \cite{croce2019minimally,croce2020reliable,li2019nattack,andriushchenko2019square,tu2019autozoom}.
}
            % Error rates on $\mathcal{D}$ for NoBox known architecture attacks with $\epsilon=.3$ and $\epsilon=.03125$}
    \end{small}
    % \vspace{-2mm}
\end{table}
\begin{table}[h]
    % \vspace{-1mm}
\begin{small}
    \centering
            \begin{tabular}{ccccccc}
            \toprule
                   Source & Attack &   VGG-16 & WR  \\
                            \midrule
                            & Clean & $11.2 \pm 0.9$  & $6.8 \pm 0.7$  \\
                            \midrule
\multirow{3}{*}{RN-18}      & MI-Attack & $71.2 \pm 1.3$  & $66.6 \pm 1.1$  \\
                            & DI-Attack & \textbf{72.6 $\pm$ 1.3}  & \textbf{73.0 $\pm$ 1.3}  \\
                            % & TID-Attack & $22.6 \pm 2.0$ & $26.6 \pm 1.9$ & $13.5 \pm 1.4$ & $22.1 \pm 2.1$ & $19.2 \pm 1.4$ \\
                            % & SGM-Attack & $68.4 \pm 1.8$ & $79.5 \pm 0.5$ & $64.3 \pm 1.6$ & $73.8 \pm 1.0$& $70.6 \pm 1.7$ \\
                            & AEG (Ours)  & \textbf{71.4 $\pm$ 3.0}  & \textbf{70.0 $\pm$ 2.5}  \\
                            \midrule
\multirow{3}{*}{DN-121}      & MI-Attack & $54.7 \pm 1.4$  & $55.5 \pm 1.3$  \\
                            & DI-Attack & $61.1 \pm 1.9 $ & $64.1 \pm 1.5$  \\
                            % & TID-Attack & $20.1 \pm 1.9$ & $22.6 \pm 2.5$ & $13.3 \pm 1.4$ & $20.9 \pm 1.6$ & $21.6 \pm 2.2$ \\
                            % & SGM-Attack & $51.6 \pm 0.7$ & $60.2 \pm 1.3$ & $52.6 \pm 0.9$ & $64.7 \pm 1.6$ & $61.4 \pm 1.3 $ \\
                            & AEG (Ours) & \textbf{69.0 $\pm$ 3.8} & \textbf{78.6 $\pm$ 2.1} \\
                           \midrule
% \multirow{5}{*}{WR}      & MI-Attack & $71.2 \pm 2.2$ & $86.0 \pm 1.7$ & \textbf{99.9 $\pm$ 0.1} & $89.0 \pm 2.6$ & $88.2 \pm 1.4$\\
%                             & DI-Attack & \textbf{75.4 $\pm$ 1.5} & \textbf{88.5 $\pm$ 2.1} & \textbf{99.9 $\pm$ 0.1} & \textbf{91.2 $\pm$ 1.6} & \textbf{91.5 $\pm$ 1.8}\\
%                             & TID-Attack & $21.9 \pm 2.2 $ & $25.2 \pm 1.7$ & $19.7 \pm 1.5$ & $21.9 \pm 1.7$ & $21.9 \pm 1.9$ \\
%                             & SGM-Attack & $69.1 \pm 2.1$ & \textbf{88.6 $\pm$ 2.0} & \textbf{99.6 $\pm$ 0.4} & \textbf{90.7 $\pm$ 1.9} & $86.8 \pm 2.2$ \\
%                             & AEG (Ours) & $40.8\pm 3.22$ & $70.6 \pm 4.9$ & $98.5 \pm 0.6$ & \textbf{88.2 $\pm$ 4.6} & \textbf{89.6 $\pm$ 1.8} \\
            \bottomrule
            \end{tabular}
            \caption{
            % Error rates on $\mathcal{D}$ for average NoBox architecture transfer attacks with $\epsilon=0.03125$}
            We now consider NoBox attacks where we do not know the architecture of the target model. For evaluation, we train $10$ instances of VGG-16 \cite{simonyan2014very}, and  Wide ResNet (WR) \cite{zagoruyko2016wide}. 
Here, we optimize the attack approaches against a single pre-trained classifier from a particular architecture and then evaluate their attack success on classifiers from distinct architectures.  
%Similar to the previous experimental setting we first randomly select a pre-trained classifier from a given source architecture. Dissimilar to the previous setting we now evaluate the adversarial examples against all other classifiers with different architectures. 
% Our findings when using ResNet-18, DenseNet-121 and the Wide ResNet as the source architecture are provided in Table 2.
When attacks are performed with a DN-121 source model, we observe that our AEG framework consistently outperforms the baselines. We hypothesize that as DN-121 can represent a relatively large hypothesis class, this leads to a particularly effective generator in the AEG framework. 
When using RN-18, we find that AEG is on par with and sometimes exceeds the state-of-the-art baselines.
% Finally, when using WR, we again obtain competitive results, except when the target model is VGG-16, which we believe is driven by the large mismatch in the underlying hypothesis classes for the WR and VGG-16 architectures.
}
            \label{q3_table}
    \end{small}
    \vspace{-2mm}
\end{table}

% \xhdr{Q3: Attacking Robust Classifiers}
% \label{q3}


%We find that the AEG adversarial examples are quite effective against vanilla adversarial training and are at par or outperform previous approaches, which matches expectations given that the saddle point of the AEG framework corresponds to attacking such a robustified classifier.
%We reconcile this fact by noting that at the saddle point the generator is optimized against the best in class classifier and this includes models robustified using PGD adversarial training. 
%On CIFAR-10 we find that TID-Attack to be the strongest adversary and that AEG attacks are less effective. 
%This is unsurprising, since ensemble adversarial training involves injecting adversarial examples from other architectures, extending the underlying hypothesis class beyond that which the generator was optimized on. %, yet the generator is optimized against a critic which never observes such adversarial examples from other architectures and consequently the generator cannot effectively attack an $f_t$ far removed from the space of functions it has trained against. 


% \begin{table*}[h]
% \vspace{-2mm}
%     \begin{small}
%     \centering
%             \begin{tabular}{cccccccc}
%             \toprule
%                   Dataset & Defence &  Clean & MI-Att$^\dag$ & DI-Att & TID-Att & SGM-Att $^\dag$ & AEG (Ours) \\
%                             \midrule
% \multirow{5}{*}{MNIST}      & $\textrm{A}_\text{ens4}$ & $0.8$ & $41.4$ & \textbf{42.7 $\pm$ 0.8} & $16.0 \pm 1.0$ & N/A & $29.2 \pm 1.4$ \\
%                             & $\textrm{B}_\text{ens4}$ & $0.7$ & \textbf{42.2} & $38.7 \pm 0.7$ & $25.8 \pm 0.4$ & N/A & $40.2 \pm 0.9$ \\
%                             & $\textrm{C}_\text{ens4}$ & $0.8$ & \textbf{73.0} & $30.0 \pm 1.5$ & $9.5 \pm 0.3$ & N/A & $37.1 \pm 0.0$ \\
%                             & $\textrm{D}_\text{ens4}$ & $1.8$ & \textbf{84.4} & $76.0 \pm 1.4$ & $81.3 \pm 0.8$ & N/A & $67.9\pm 1.6$ \\
%                             & Madry-Adv & $0.8$ & $2.0$ & \textbf{3.1 $\pm$ 0.2} & $2.5 \pm 0.2$ & N/A & \textbf{3.0 $\pm$ 0.2}\\
%                             \midrule
% \multirow{5}{*}{CIFAR-10}   & $\textrm{RN-18}_\text{ens3}$ & $16.8$ & $17.6$ & $21.6 \pm 0.8$& \textbf{33.1 $\pm$ 1.4} & $19.9$  & $19.5 \pm 0.0$ \\
%                             & $\textrm{WR}_\text{ens3}$ & $12.8$ & $18.4$ & $ 20.6 \pm 1.0 $ & \textbf{28.8 $\pm$ 0.8} & $18.0$ & $15.2 \pm 0.0$ \\
%                             & $\textrm{DN-121}_\text{ens3}$ & $21.5$ & $20.3$ & $ 22.7 \pm 1.1 $ & \textbf{31.3 $\pm$ 0.3} &$21.9$ & $19.9 \pm 0.0$ \\
%                             & $\textrm{Inc-V3}_\text{ens3}$ & $14.8$ & $19.5$ & \textbf{42.2 $\pm$ 1.3}* & $30.2 \pm 0.6^*$ & $35.5$* & $23.0 \pm 0.0$ \\
%                             & Madry-Adv & $12.9$ & $17.2$  & $16.6 \pm 0.2$ & $16.6 \pm 0.5$ & $16.0$ & \textbf{18.7 $\pm$ 0.0}\\
%             \bottomrule
%             \end{tabular}
%             \caption{ \small
%             We now test the ability of our AEG framework to attack target models that have been robustified using adversarial and ensemble adversarial training \cite{madry2017towards,tramer2017ensemble}. 
% For evaluation against PGD adversarial training, we use the public models as part of the MNIST and CIFAR-10 adversarial examples challenge. 
% \footnote{\url{https://github.com/MadryLab/[dataset]_challenge}, for \texttt{[dataset]} in $\{\texttt{cifar10},\texttt{mnist}\}$.
% Note that our threat model is more challenging than these challenges as we use non-robust source models.
% }
% For ensemble adversarial training, we follow the approach of \citet{tramer2017ensemble} (see Appendix \ref{appendix:ens_adv_training}). 
% We report our results in Table 3 and average the result of stochastic attacks over $5$ runs. 
% We find that the AEG adversarial examples are able to succesfully models robustified through ensemble adversarial training. Specifically, AEG is competitive with most baselines but falls short of the powerful MI-Attack on the MNIST dataset. On CIFAR-10, we find that DI-Attack and TID-Attack to be the strongest and that AEG attacks are less effective. This is unsurprising, due to the inherent difficulties in saddle point optimization~\citep{gidel2019variational,Berard2020A} and since ensemble adversarial training involves injecting adversarial examples from other architectures, extending the underlying hypothesis class beyond which the generator was optimized on. Thus the chosen representative classifier classifier is suboptimal compared to representational power of the target model which constitutes an ensemble of architectures. Against PGD adversarial training, we observe that AEG adversarial examples matches SOTA for MNIST while exceeds it on CIFAR-10. We reconcile this result by recalling the saddle point of the AEG framework corresponds to attacking the strongest robustified classifier which includes classifiers robustified via PGD adversarial training.
% }
%             % Error rates on $\mathcal{D}$ for NoBox known architecture attacks against Adversarial Training and Ensemble Adversarial Training. ${}^*$ Attacks were done using WR. ${}^\dag$ Deterministic attack.}
%     \end{small}
%     \vspace{-5mm}
% \end{table*}

    
    
    
    
    %%%%%%% Old Table 1:
    \cut{
\begin{table}[ht]
    \label{q1_table}
    \centering
          
            \begin{tabular}{cccccc}
            \toprule
                   &            \multicolumn{2}{c}{MNIST}  & \multicolumn{2}{c}{CIFAR-10}\\
                   Threat Model & Attack &  $l_{\infty}$ \ & $l_2$ \ &  $l_{\infty}$ &  $l_2$ \\
                    \midrule
\multirow{4}{*}{Whitebox} & AutoAttack* & $84.41 \pm 5.06$ & $19.59 \pm 4.03 $ & $91.02 \pm 1.86$ & - \\
                   & APGD-CE & $95.81 \pm 1.85 $ & $24.32 \pm 5.52 $ & $97.48 \pm 0.74$ & - \\
                   & APGD-DLR & $83.91 \pm 5.37 $ & $20.14 \pm 4.29 $ & $90.67 \pm 2.12$ & - \\
                   & FAB & $5.36 \pm 2.19$ & $6.18 \pm 2.99 $ & $10.42 \pm 1.70$ & - \\
                   \midrule 
\multirow{3}{*}{Blackbox-query} & Square & $60.86 \pm 10.25$ & $13.18 \pm 4.30 $ & $21.92 \pm 2.82$ & - \\
                   & AutoZoom-BiLIN & - & $10.40 \pm 3.07 $ & - & -\\
                   &$\mathcal{N}$-Attack & $9.45 \pm 3.16 $ & - & $56.74 \pm 8.91$ & - \\
                   \midrule 
\multirow{4}{*}{\shortstack{Non-Interactive \\ Blackbox}}& MI-Attack & $93.73 \pm 1.11 $ & $82.24 \pm 1.42 $ & \textbf{99.96} $\pm 0.12$ & - \\
                    & DI-Attack & $90.82 \pm 2.77 $ & $12.82 \pm 5.40 $ & $45.23 \pm 2.91$ & - \\
                    & TI-Attack & - & - & - & - \\
                    & SGM-Attack & - & - & \textbf{99.83} $ \pm 0.32$ & - \\
                    & Ours (Transfer) & \textbf{95.78 $\pm$ 2.76} & \textbf{97.00(not anymore)\%} & - & -\\
            \bottomrule
            \end{tabular}
            \caption{Test error rates for average blackbox transfer over architectures at $\epsilon=0.3$ ($\ell_2, \epsilon = 1.5$ )(higher is better)}
    \end{table}
}


==> MAIS2020/intro.tex <==
% \section{Introduction}

\xhdr{Introduction}
Adversarial attacks on deep neural nets expose critical vulnerabilities in traditional machine learning systems \citep{moosavi2016deepfool,athalye2018synthesizing,sun2018survey,bose2018adversarial}. 
In order to develop better machine learning models robust to such adversarial attacks, it is imperative to improve our theoretical understanding of different attack strategies. 
While there has been considerable progress in understanding the theoretical underpinnings of adversarial attacks in relatively permissive settings (e.g. {\em whitebox} adversaries \citep{madry2017towards}), there remains a substantial gap between theory and practice in more demanding and realistic threat models.

In this work, we provide a theoretical framework for understanding and analyzing adversarial attacks in the highly-challenging {\em \textbf{No}n-interactive black\textbf{Box} adversary} (NoBox) setting,
where the attacker has no direct access, including input-output queries, to the target classifier it seeks to fool.
Instead, the attacker must generate attacks by optimizing against some representative classifiers, which are assumed to come from a similar hypothesis class as the target, before applying these attacks in a single attempt against the target classifier.

The NoBox setting is a much more challenging setting than more traditional threat models, yet it is representative of many real-world attack scenarios, where the attacker cannot interact with the target model \citep{carlini2019evaluating}. 
Indeed, this setting---as well as the general notion of transferring attacks between classifiers---has generated an increasing amount of empirical interest \citep{dong2019evading,liu2016delving,xie2019improving,wu2020skip}, though the field currently lacks the necessary theoretical foundations to understand the feasibility of such attacks.  

\xhdr{Present Work}
To address this theoretical gap, we cast NoBox attacks as a kind of {\em adversarial examples game} (AEG).
In this game, an attacker generates adversarial examples to fool a representative classifier from a given hypothesis class, while the classifier itself is trained to detect the correct labels from the adversarially generated examples. Our first main result shows that the Nash equilibrium of an AEG leads to a distribution of adversarial examples effective against {\em any} classifier from the given function class.
More formally, this adversarial distribution is guaranteed to be the most effective distribution for attacking the hardest-to-fool classifiers within the hypothesis class, providing a worst-case guarantee for attack success against an arbitrary target. 
We further show that this optimal adversarial distribution admits a natural interpretation as being the distribution that maximizes a form of restricted conditional entropy over the target dataset, and we provide detailed analysis on simple parametric models to illustrate the characteristics of this optimal adversarial distribution. Note that while AEGs are latent games~\citep{gidel2020minimax}, they are distinct from the popular generative adversarial networks (GANs)~\citep{goodfellow2014generative}. In AEGs, there is \emph{no} discrimination task between two datasets (generated one and real one); instead, there is a standard supervised (multi-class) classification task on an adversarial dataset.

Empirical results on standard benchmarks using models that directly instantiate the AEG framework show that we can achieve competitive performance---compared to existing heuristic approaches---in the NoBox setting while maintaining a firm theoretical grounding. 
In particular, we find that our framework can achieve state-of-the-art performance in many settings (e.g., attacking a held-out classifier with DenseNet architectures on CIFAR-10), while remaining highly competitive in others. 




==> no_box_attack.tex <==
\section{Attacking in the wild: Nobox attack}
The modeling framework is the following. Given an input datapoint $x$ its associated output is sampled from the probability distribution $p=\sP(y|x)$. An adversarial example with no assumption on the classifier can be seen as a pertubation of $x$ that attack the probability distribution of the data. Formally, given a loss function, $\ell: \Delta \gY \times \Delta \gY \to \sR$,
\begin{equation}
    x_{adv} \in \arg \max_{\|x'-x\| \leq \epsilon} \ell(p,\sP(y|x'))
\end{equation}
\ggi{Check related work regarding robust learning}

finite dataset, epsilon coverage of the real support. Check robust optimization theory. 

\ggi{Maybe more general we can start without talking about a class of function would be even stronger maybe}

Given a class of function $\mathcal{F}$ -- e.g., a given architecture for the classifier -- we aim at being able to attack any function within this class.

\begin{equation}\label{eq:no_box_attack}
    x_{adv} \in \arg \max_{\|x'-x\| \leq \epsilon} \ell_f(x',y)
\end{equation}
We want to learn a conditional distribution of adversarial examples $p_{adv}(\cdot|x)$ respecting the proximity constraint in~\eqref{eq:opt_attack}.

This way we can attack a class of function. 

The choice of learning a distribution instead of a deterministic mapping will be further motivated and discussed in Section~\ref{sec:adv_example_game}

==> setting.tex <==
\section{No box attack}
One question is, can we switch $\min$ and $\max$? 

If we are in the non-parametric case, we have for a given distribution $(x,y) \sim data$
\begin{equation}
    \min_{f \in \ell_2} \max_{g \in \mathcal{G}}\mathbb{E}_{(x,y) \sim data, x' \sim g(x'|x)}[ \ell(f(g(x)),y)] =  \min_{f \in \ell_2}  \max_{d_x(p_g,data) \leq \delta} \mathbb{E}_{(x',y) \sim p_g}[ \ell(f(x'),y)]
\end{equation}
This problem is convex-concave (if $ell$ is convex) and the constraints sets are convex and compact (actually only compact with a finite dataset). Thus, by Sion's minimax theorem we have the existence of an equilibrium. 

Moreover, we know that if $\mathbb E [y|x] \in \ell_2$, we have,
\begin{equation}
    f(x) := \mathbb E [y|x]
\end{equation}
(only true with a consistent loss, but any standard loss is consistent so anyway...).
\begin{equation}
     \max_{g }\min_{f }\mathbb{E}_{(x,y) \sim data, x' = g(x)}[ \ell(f(g(x)),y)] = \max_{d_x(p_g,data) \leq \delta} \mathbb{E}_{(x,y) \sim p_g}[ \ell(\mathbb E[y|x'],y)]
\end{equation}
where $d_x$ is a distance on the marginalization of the distributions. If we assume that $\ell$ is bounded (true for square loss) by $B$, then we have 
\begin{equation}
      |\max_{d_x(p_g,data) \leq \delta} \mathbb{E}_{(x,y) \sim p_g}[ \ell(\mathbb E[y|x'],y)] - \mathbb{E}_{(x,y) \sim data}[ \ell(\mathbb E[y|x],y)]| \leq \delta B
\end{equation}
